WrappingNet: Mesh Autoencoder via Deep Sphere Deformation

There have been recent efforts to learn more meaningful representations via fixed length codewords from mesh data, since a mesh serves as a complete model of underlying 3D shape compared to a point cloud. However, the mesh connectivity presents new difficulties when constructing a deep learning pipeline for meshes. Previous mesh unsupervised learning approaches typically assume category-specific templates, e.g., human face/body templates. It restricts the learned latent codes to only be meaningful for objects in a specific category, so the learned latent spaces are unable to be used across different types of objects. In this work, we present WrappingNet, the first mesh autoencoder enabling general mesh unsupervised learning over heterogeneous objects. It introduces a novel base graph in the bottleneck dedicated to representing mesh connectivity, which is shown to facilitate learning a shared latent space representing object shape. The superiority of WrappingNet mesh learning is further demonstrated via improved reconstruction quality and competitive classification compared to point cloud learning, as well as latent interpolation between meshes of different categories.

==> 4_framework.tex <==
We now describe the details of the encoder and decoder modules, before discussing our deformation backbone, which is used to perform all wrapping-related operations on the meshes.
\subsection{UnWrapping-based Encoder}
\label{sec:encoder}
In the encoder, the initial feature extractor (FE) uses a SubdivNet backbone to generate a feature map on the faces of the base mesh. This alternates between face convolutions and subdivision pooling which pools 4 faces to 1 face (we use average pooling), down to the base mesh. This allows for hierarchical feature processing of the original mesh. To generate a single latent code, the feature map is processed by a shared MLP with global pooling across the faces. Global pooling ensures that the same size latent code is generated across all meshes in the entire dataset. 

As mentioned previously, if the codeword $\cv$ was accompanied by the base mesh, it would fail to fully capture the global shape information. To fully inject the global shape information into the codeword and disentangle it from the base mesh, we introduce a novel \emph{UnWrapping} step. This is achieved by using the deformation backbone (Sec.~\ref{sec:deformation_backbone} \JA{to fix label}) to deform the base mesh into a sphere mesh; we choose a sphere due to its desirable rotation equivariance properties. The deformed sphere mesh is then matched with a fixed grid of points on the sphere defined by the Fibonacci lattice \cite{fibonaccilattice}, which we refer to as the \textit{sphere grid}. The objective of the matching step is twofold: i) it projects the deformed sphere mesh vertices perfectly onto a 3D sphere, and ii) reindexes the base graph to be aligned with the fixed ordering of the sphere grid. The matching method used is described in detail in the supplementary. What is then sent to the decoder is the latent code $\cv$ and the reindexed base graph $G$.



\subsection{Wrapping-based Decoder}
\label{sec:decoder}
 The latent code and base graph can be used by the decoder to form an initial sphere mesh by combining the base graph with the vertices of the sphere grid, which is the same sphere grid as the one in the encoder. Since the decoder is forced to reconstruct the mesh from a canonical sphere geometry (with base graph connectivity), the codeword is forced to learn the global shape when the architecture is trained in an end-to-end manner. 

The proposed decoder, also shown in Fig.~\ref{fig:E2E}, consists of two \emph{Wrapping} stages. Architecturally, the first stage uses the same deformation backbone as the UnWrapping step. It consumes the initial sphere mesh, along with the codeword which is copied onto each of the sphere mesh's faces. The output of this stage is passed to the second Wrapping step, which uses the deformation backbone architecture interleaved with unpooling layers that subdivide each face into four. This simultaneously upsamples the first Wrapping output to the original resolution and refines the vertex positions in order to produce the final reconstructed mesh. 



\subsection{Deformation Backbone}
\label{sec:deformation_backbone}
We now describe our novel deformation backbone, which is used in the unwrapping step in the encoder, and both wrapping steps in the decoder. The deformation backbone is comprised of alternating face convolution (FaceConv) layers\footnote{From SubdivNet \cite{subdivnet}. More details in supplementary.} and our novel \textit{Face2Node} layers. At a high level, the FaceConv layers are face feature-based, but in order to deform a mesh, we need to perform node-wise updates of the vertex positions in a differentiable manner; this necessitates a face to node conversion of information.

The Face2Node module consumes a mesh along with face features $\Fv$ and i) predicts differential vertex position updates, and ii) optionally updates the face features. 

Let $v$ be a node we are updating, $\mathcal{N}_v$ denote the faces that node $v$ is a part of, and let $\Fv_i$ denote the $i$-th face's feature, and suppose $i \in \mathcal{N}_v$, \ie, $v$ is a node of face $i$. Face2Node first creates a new feature for face $i$ relative to $v$ by concatenating edge vectors of face $i$ to $\Fv_i$, \ie, if $\xv\ssi{0}, \xv\ssi{1}, \xv\ssi{2}$ are the three vertex positions of face $i$, its edge vectors are $\ev\ssi{k} = \xv\ssi{k+1 \mod 3}-\xv\ssi{k}$, $k \in \{0,1,2\}$. We ensure the edge vectors are concatenated in an order-equivariant manner, \ie, if the local node ordering \textit{within a face} is permuted, the concatenation order permutes accordingly. Since nodes within a face are ordered so that normals point outward, this can be achieved by fixing a relative starting index. We set this to be the node index within face $i$ that $v$ happens to be, denoted as $j(v)$. The concatenated feature for face $i$ relative to $v$ is given by
\begin{equation}
    \fv_i\ssi{j(v)} = \Fv_i || \ev\ssi{j(v)}||\ev\ssi{j(v)+1 \mod 3}||\ev\ssi{j(v)+2 \mod 3}
\end{equation}
where $||$ denotes concatenation. A figure illustrating this process can be found in Fig.~\ref{fig:Face2NodeOperational}. As shown in Fig.~\ref{fig:Face2Node}, Face2Node then updates the concatenated face features (for all faces in $\mathcal{N}_v$) using a shared MLP, \ie, $\gv_i\ssi{j(v)} = \mathrm{MLP}(\fv_i\ssi{j(v)})$. The differential position update for node $v$ is the average of the first 3 components of $\gv_i\ssi{j(v)}$, averaged over $\mathcal{N}_v$. 

Then the differential position update of $v$ is $\Delta_v = \frac{1}{|\mathcal{N}_v|} \sum_{i \in \mathcal{N}_v}  \gv_i\ssi{j(v)}\text{[0:3]}$, and
the node position is updated as $\xv_v \leftarrow \xv_v + \Delta_v$. The face features are then updated simply by averaging over all three versions of the remaining entries $\gv_i\ssi{j(v)}\text{[3:]}$ for the $i$-th face, $\Fv_i \leftarrow \frac{1}{3}(\gv_i\ssi{0}\text{[3:]}+\gv_i\ssi{1}\text{[3:]}+\gv_i\ssi{2}\text{[3:]})$,
which ensures the features on the face remain invariant to the order of its nodes. This is important because the FaceConv layers are designed to be agnostic to specific node orderings.

\begin{figure}
    \centering
    \includegraphics[width=0.25\linewidth]{diagrams/Face2NodeOperational.png}
    \caption{Aggregation of neighboring faces around node $v$. In this example, for face $i$, the edge vectors are concatenated in the blue, green, red order. Note that the direction of the nodes in each face are predefined for the normals to have a consistent direction.}
    \label{fig:Face2NodeOperational}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{diagrams/Face2Node_new.png}
    \caption{\textbf{Face2Node} module. Face-wise MLP updates face features, which are used to update vertex position and face features.}
    \label{fig:Face2Node}
\end{figure}

\begin{table*}[htbp]
  \centering\scriptsize
  \caption{Average classification performance from test latent representations using SVM with 5-fold cross-validation.}
    \begin{tabular}{c||ccc|ccc|ccc}
    \hline
    Dataset & \multicolumn{3}{c|}{SHREC11} & \multicolumn{3}{c|}{Manifold10} & \multicolumn{3}{c}{Mainfold40} \bigstrut\\
    \hline
    Metric & Acc.  & Prec. & Recall & Acc.  & Prec. & Recall & Acc.  & Prec. & Recall \bigstrut\\
    \hline
    \hline
    FoldingNet & 99.4\% & 0.995 & 0.995 & \textbf{91.0\%} & 0.901 & 0.893 & 82.5\% & 0.756 & 0.678 \bigstrut[t]\\
    TearingNet & \textbf{99.8\%} & \textbf{0.998} & \textbf{0.998} & 90.8\% & 0.901 & 0.892 & 82.9\% & 0.750 & 0.664 \\
    WrappingNet & 99.1\% & 0.991 & 0.991 & 90.9\% & \textbf{0.908} & \textbf{0.902} & \textbf{83.3\%} & \textbf{0.778} & \textbf{0.730} \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:class_results}%
  \vspace{-10pt}
\end{table*}%

\subsection{Permutation Invariance and Equivariance}
An important aspect of WrappingNet is that the model should not be affected by changes in the indexing of the vertices or faces. Overall, a forward pass through the entire WrappingNet is permutation-invariant, in that if the input mesh's nodes are permuted, the decoder will still output the same shape in a fixed ordering. To see why, we first look at the deformation backbone, which achieves permutation equivariance to both face and vertex order due to the design of the FaceConv layers (details in Supplementary) as well as the Face2Node layers, which either avoid order-specific processing or ensure that any operations dependent on order are equivariant. 

For the encoder, the SubdivNet-based feature extractor is permutation-equivariant, and both subsequent branches (base graph branch and the codeword branch) are permutation-invariant. For the codeword branch, this is achieved via global pooling. For the base graph branch, the deformation backbone is permutation-equivariant, as mentioned above. At the matching stage, we first note that the matching method used (in supplementary) depends only on the node positions; even if the UnWrapping output is permuted, the same set of points from the sphere grid will be selected. Since the sphere grid is in a \textit{fixed} ordering, the base graph (which is permuted in the sphere grid's order) is invariant to the matching step's input. 

At the decoder, the two wrapping stages are both based on the deformation backbone, and hence achieve permutation-equivariance. Since the encoder is permutation-invariant, however, the end-to-end model remains permutation-invariant.

% \subsection{Training Details}
% \label{sec:training}
% Our proposed architecture WrappingNet is trained in two distinct stages. In the first training stage, which we refer to as pretraining, the deformation backbone in the UnWrapping step is pretrained by providing base mesh examples as input and supervision through a Chamfer loss with random point clouds sampled from the unit sphere.

% In the second training stage, during the end-to-end training of the full architecture, the weights of the UnWrapping step are fixed, and the predicted sphere positions are index-matched with a canonical sphere grid defined by the Fibonacci lattice \cite{fibonaccilattice}, of the same size as the base mesh. During this training process, we enforce a loss at the output of both Wrapping steps. Due to the subdivision mesh structure, we maintain vertex correspondences between the input mesh and outputs of both Wrapping stages. Hence, we supervise a vertex-to-vertex L2 loss between both output lists of positions and the input mesh vertex positions.

% The index-matching is performed using the Sinkhorn algorithm \cite{cuturi2013sinkhorn, peyre2019computational} with Euclidean distance cost between each pair of 3D points. Further details regarding the index matching can be found in the supplementary material. 

% One important concept to highlight is that the face features that propagate throughout the model are ensured to be local to the region on the mesh the face resides on and does have knowledge of the global location. In this sense, the SphereNet locally deforms regions on the base mesh to a sphere, and the decoder locally deforms the sphere mesh back into the original shape. The global orientation of the shape is still kept within the sphere. In other words, while the model is not guaranteed to be equivariant to 3D rotations, the use of local feature processing helps to achieve this capability. \ML{Not so sure about this paragraph in terms of content and placement.}



